Improving Tree Probability Estimation with Stochastic Optimization and Variance Reduction

Probability estimation of tree topologies is one of the fundamental tasks in phylogenetic inference. The recently proposed subsplit Bayesian networks (SBNs) provide a powerful probabilistic graphical model for tree topology probability estimation by properly leveraging the hierarchical structure of phylogenetic trees. However, the expectation maximization (EM) method currently used for learning SBN parameters does not scale up to large data sets. In this paper, we introduce several computationally efficient methods for training SBNs and show that variance reduction could be the key for better performance. Furthermore, we also introduce the variance reduction technique to improve the optimization of SBN parameters for variational Bayesian phylogenetic inference (VBPI). Extensive synthetic and real data experiments demonstrate that our methods outperform previous baseline methods on the tasks of tree topology probability estimation as well as Bayesian phylogenetic inference using SBNs.

==> bn-example.tex <==
\input{rooted_tree}
\tikzstyle{fakenode} = [obs, fill=gray!10, draw=gray, densely dashed]
\tikz[scale=0.7]{
  \begin{scope}[xscale=0.8, yscale=0.8, transform shape, rounded corners]
  \node[leaf, xshift=7cm, yshift=3.5cm] (A) {$O_1$};
  \node[leaf, xshift=7cm, yshift=2.5cm] (B) {$O_2$};
  \node[leaf, xshift=7cm, yshift=1.5cm] (C) {$O_3$};
  \node[leaf, xshift=7cm, yshift=0.5cm] (D) {$O_4$};
  \node[leaf, xshift=7cm, yshift=-0.5cm] (E) {$O_5$};
  \node[leaf, xshift=7cm, yshift=-1.5cm] (F) {$O_6$};
  \node[leaf, xshift=7cm, yshift=-2.5cm] (G) {$O_7$};
  \node[leaf, xshift=7cm, yshift=-3.5cm] (H) {$O_8$};
  \node[clade, left=of A, yshift=-0.5cm] (C4) {\scalebox{1.2}{$C_4$}};
  \node[clade, left=of D, yshift=-0.5cm] (C6) {\scalebox{1.2}{$C_6$}};
  \node[clade, left=of F, yshift=-0.5cm] (C7) {\scalebox{1.2}{$C_7$}};
  \node[clade, left=of C4, xshift=-2cm, yshift=-1.125cm] (C2) {\scalebox{1.2}{$C_2$}};
  \node[clade, left=of C6, yshift=0.75cm] (C5) {\scalebox{1.2}{$C_5$}};
  \node[clade, left=of C7, xshift=-2cm, yshift=-0.75cm] (C3) {\scalebox{1.2}{$C_3$}};
  \node[clade, left=of C2, yshift=-2.3125cm] (C1) {\scalebox{1.2}{$C_1$}};
  \end{scope}
  \squaredge[thick] {C1}{C2, C3};
  \squaredge[thick] {C2}{C4, C5};
  \squaredge[thick] {C4}{A, B};
  \squaredge[thick] {C5}{C, C6};
  \squaredge[thick] {C6}{D, E};
  \squaredge[thick] {C3}{C7, H};
  \squaredge[thick] {C7}{F, G};
    
  \begin{scope}[xscale=0.6, yscale=0.6, transform shape, xshift=23.5cm, yshift=5cm]
    \node[fakenode, xshift=5cm] (SP8) {\scalebox{1.8}{$1$}};
    \node[fakenode, below=of SP8, yshift=0.3cm] (SP9) {\scalebox{1.8}{$2$}};
    \node[obs, left=of SP8, xshift=-1.5cm, yshift=-1.5cm] (SP4) {\scalebox{1.2}{$\dfrac{1}{2}$}};
    \node[obs, below=of SP4, yshift=-0.1cm] (SP5) {\scalebox{1.4}{$\dfrac{3}{45}$}};
    \node[fakenode, below=of SP9, yshift=0.3cm] (SP10) {\scalebox{1.8}{$3$}};
    \node[obs, below=of SP10, yshift=0.3cm] (SP11) {\scalebox{1.2}{$\dfrac{4}{5}$}};
    \node[fakenode, below=of SP11, yshift=0.3cm] (SP12) {\scalebox{1.8}{$6$}};
    \node[fakenode, below=of SP12, yshift=0.3cm] (SP13) {\scalebox{1.8}{$7$}};
    \node[obs, below=of SP5, yshift=-0.6cm] (SP6){\scalebox{1.2}{$\dfrac{6}{7}$}};
    \node[fakenode, below=of SP6, yshift=-0.3cm] (SP7) {\scalebox{1.8}{$8$}};
    \node[fakenode, below=of SP13, yshift=0.3cm] (SP14) {\scalebox{1.8}{$8$}};
    \node[fakenode, below=of SP14, yshift=0.3cm] (SP15) {\scalebox{1.8}{$8$}};
    \node[obs, left=of SP4, xshift=-1.5cm, yshift=-1.5cm] (SP2) {\scalebox{1.4}{$\dfrac{12}{345}$}};
    \node[obs, below=of SP2, yshift=-1.6cm] (SP3) {\scalebox{1.4}{$\dfrac{67}{8}$}};
    \node[obs, left=of SP2, xshift=-1.5cm, yshift=-2.0cm] (SP1) {\scalebox{1.6}{$\dfrac{12345}{678}$}};
    
    \annotatededge[densely dashed, gray!50] {}{}{SP4}{SP8, SP9};
    \annotatededge[densely dashed, gray!50] {}{}{SP5}{SP10};
    \edge{SP5}{SP11};
    \annotatededge[densely dashed, gray!50] {}{}{SP6}{SP12, SP13};
    \annotatededge[densely dashed, gray!50] {}{}{SP7}{SP14, SP15};
    \edge{SP2}{SP4, SP5};
    \edge{SP3}{SP6};
    \annotatededge[densely dashed, gray!50] {}{}{SP3}{SP7};
    \edge{SP1}{SP2, SP3};
  \end{scope}
  
  \node[left=0.5cm of SP1, xshift=-1.05cm] (Arrow) {};
  \draw[<->, >=stealth, thick] (Arrow) -- + (1, 0);
  }

==> bn-reversed.tex <==
\input{rooted_tree}
\tikz[scale=0.65]{
  \begin{scope}[xscale=0.52, yscale=0.52, transform shape]
  \node[obs](S1){\scalebox{1.8}{$S_1$}};
  \node[obs, right=of S1, xshift=0.75cm, yshift=1.8cm](S2){\scalebox{1.8}{$S_2$}};
  \node[obs, right=of S1, xshift=0.75cm, yshift=-1.8cm](S3){\scalebox{1.8}{$S_3$}};
  \node[obs, right=of S2, xshift=0.75cm, yshift=1.8cm](S4){\scalebox{1.8}{$S_4$}};
  \node[obs, right=of S2, xshift=0.75cm, yshift=-0.6cm](S5){\scalebox{1.8}{$S_5$}};
  \node[obs, right=of S3, xshift=0.75cm, yshift=0.6cm](S6){\scalebox{1.8}{$S_6$}};
  \node[obs, right=of S3, xshift=0.75cm, yshift=-1.8cm](S7){\scalebox{1.8}{$S_7$}};
  \node[obs, right=of S4, xshift=0.75cm, yshift=1.8cm](S8){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S4, xshift=0.75cm, yshift=0.25cm](S9){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S5, xshift=0.75cm, yshift=1.05cm](S10){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S5, xshift=0.75cm, yshift=-0.45cm](S11){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S6, xshift=0.75cm, yshift=0.45cm](S12){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S6, xshift=0.75cm, yshift=-1.05cm](S13){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S7, xshift=0.75cm, yshift=-0.25cm](S14){\scalebox{1.8}{$\cdots$}};
  \node[obs, right=of S7, xshift=0.75cm, yshift=-1.8cm](S15){\scalebox{1.8}{$\cdots$}};
  \edge{S1}{S2, S3} ;
  \edge{S2}{S4, S5} ;
  \edge{S3}{S6, S7} ;
  \edge{S4}{S8, S9};
  \edge{S5}{S10, S11};
  \edge{S6}{S12, S13};
  \edge{S7}{S14, S15};
  \path (S1) edge [->, >={triangle 45}, bend right=10, dashed]  (S5);
  \path (S1) edge [->, >={triangle 45}, bend right=-30, dashed]  (S4);
  \path (S1) edge [->, >={triangle 45}, bend right=-10, dashed]  (S6);
  \path (S1) edge [->, >={triangle 45}, bend right=30, dashed]  (S7);
  \path (S2) edge [->, >={triangle 45}, bend right=5, dashed]  (S9);
  \path (S2) edge [->, >={triangle 45}, bend right=-30, dashed]  (S8);
  \path (S2) edge [->, >={triangle 45}, bend right=-5, dashed]  (S10);
  \path (S2) edge [->, >={triangle 45}, bend right=20, dashed]  (S11);
  \path (S3) edge [->, >={triangle 45}, bend right=-20, dashed]  (S12);
  \path (S3) edge [->, >={triangle 45}, bend right=5, dashed]  (S13);
  \path (S3) edge [->, >={triangle 45}, bend right=-5, dashed]  (S14);
  \path (S3) edge [->, >={triangle 45}, bend right=20, dashed]  (S15);
  \end{scope}
  
  \begin{scope}[xscale=0.52, yscale=0.52, transform shape, xshift=16cm, yshift=-1cm]
  \node[obs, yshift=4cm] (T1SP1) {\scalebox{1.2}{$\dfrac{ABC}D$}};

  \node[obs, right=of T1SP1, xshift=0.5cm, yshift=1.1cm](T1SP2){\scalebox{1.2}{$\dfrac{A}{BC}$}};
  \node[obs, right=of T1SP1, xshift=0.7cm, yshift=-1.1cm, fill=gray!10, draw=gray, densely dashed](T1SP3){\scalebox{1.8}{$D$}};
  \node[obs, right=of T1SP2, xshift=0.5cm, yshift=1.1cm, fill=gray!10, draw=gray, densely dashed](T1SP4) {\scalebox{1.8}{$A$}};
  \node[obs, right=of T1SP2, xshift=0.4cm, yshift=-0.35cm](T1SP5) {\scalebox{1.2}{$\dfrac{B}C$}};
  \node[obs, right=of T1SP3, xshift=.75cm, yshift=0.35cm, fill=gray!10, draw=gray, densely dashed] (T1SP6) {\scalebox{1.8}{$D$}};
  \node[obs, right=of T1SP3, xshift=.75cm, yshift=-1.1cm, fill=gray!10, draw=gray, densely dashed] (T1SP7) {\scalebox{1.8}{$D$}};
    
  \edge{T1SP1}{T1SP2} 
  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{1.0}{T1SP1}{T1SP3};
  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{1.0}{T1SP2}{T1SP4};
  \edge{T1SP2}{T1SP5};
  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{1.0}{T1SP3}{T1SP6};
  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{1.0}{T1SP3}{T1SP7};
  
  
  \node[obs, yshift=-2.5cm] (T2SP1) {\scalebox{1.2}{$\dfrac{AB}{CD}$}};
  \node[obs, right=of T2SP1, xshift=0.5cm, yshift=1.1cm] (T2SP2) {\scalebox{1.2}{$\dfrac{A}{B}$}};
  \node[obs, right=of T2SP1, xshift=0.5cm, yshift=-1.1cm] (T2SP3) {\scalebox{1.2}{$\dfrac{C}{D}$}};
  \node[obs, right=of T2SP2, xshift=0.75cm, yshift=1.1cm, fill=gray!10, draw=gray, densely dashed] (T2SP4) {\scalebox{1.8}{$A$}};
  \node[obs, right=of T2SP2, xshift=0.75cm, yshift=-0.4cm, fill=gray!10, draw=gray, densely dashed] (T2SP5) {\scalebox{1.8}{$B$}};
  \node[obs, right=of T2SP3, xshift=0.75cm, yshift=0.4cm, fill=gray!10, draw=gray, densely dashed] (T2SP6) {\scalebox{1.8}{$C$}};
  \node[obs, right=of T2SP3, xshift=0.75cm, yshift=-1.1cm, fill=gray!10, draw=gray, densely dashed] (T2SP7) {\scalebox{1.8}{$D$}}; 
  
  \edge{T2SP1}{T2SP2, T2SP3};
  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{1.0}{T2SP2}{T2SP4};
  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{1.0}{T2SP2}{T2SP5};
  \annotatededge[densely dashed, gray!50]{pos=0.3, above=2pt}{1.0}{T2SP3}{T2SP6};
  \annotatededge[densely dashed, gray!50]{pos=0.3, below=1pt}{1.0}{T2SP3}{T2SP7};
  
  \end{scope}   

  \begin{scope}[xscale=0.52, yscale=0.52, transform shape, yshift=-1cm, xshift=30cm]
  \node[yshift=2.2cm] (T1S1) {};
  \node[left=2.5cm of T1S1, xshift=-2cm, yshift=1.6cm] (T1Arrow) {};
  \draw[<->, >=stealth, thick] (T1Arrow) -- +(1.5,0);
  \node[right=of T1S1, xshift=0.5cm, yshift=3.2cm](T1S2) {};
  \node[leaf, right=of T1S1, xshift=3.48cm] (T1D) {\scalebox{1.4}{$D$}};
  \node[leaf, right=of T1S2, xshift=1.8cm, yshift=0.75cm] (T1A) {\scalebox{1.4}{$A$}};
  \node[right=of T1S2, xshift=0.5cm, yshift=-1.2cm] (T1S3) {};
  \node[leaf, right=of T1S3, yshift=0.6cm] (T1B) {\scalebox{1.4}{$B$}};
  \node[leaf, right=of T1S3, yshift=-0.6cm] (T1C) {\scalebox{1.4}{$C$}};
  \csquaredge[thick]{T1S1}{T1S2}
  \csquaredgeleaf[thick] {T1S1}{T1D};
   \csquaredgeleaf[thick] {T1S2}{T1A};
  \csquaredge[thick]{T1S2}{T1S3};
  \csquaredgeleaf[thick]{T1S3}{T1B, T1C};
  
  
  \node[yshift=-2.5cm] (T2S1) {};
  \node[left=2.5cm of T2S1, xshift=-2cm] (T2Arrow) {};
  \draw[<->, >=stealth, thick] (T2Arrow) -- +(1.5, 0);
  \node[right=of T2S1, xshift=0.75cm, yshift=1.25cm] (T2S2) {};
  \node[right=of T2S1, xshift=0.75cm, yshift=-1.25cm] (T2S3) {};
  \node[leaf, right=of T2S2, xshift=1.45cm, yshift=0.75cm] (T2A) {\scalebox{1.4}{$A$}};
  \node[leaf, right=of T2S2, xshift=1.45cm, yshift=-0.6cm] (T2B) {\scalebox{1.4}{$B$}};
  \node[leaf, right=of T2S3, xshift=1.45cm, yshift=0.6cm] (T2C) {\scalebox{1.4}{$C$}};
  \node[leaf, right=of T2S3, xshift=1.45cm, yshift=-0.75cm] (T2D) {\scalebox{1.4}{$D$}};
  \csquaredge[thick]{T2S1}{T2S2, T2S3};
  \csquaredgeleaf[thick]{T2S2}{T2A, T2B};
  \csquaredgeleaf[thick]{T2S3}{T2C, T2D};
  \end{scope}
  
%
%
%  \node[xshift=1.4cm, yshift=-2.5cm]  {$(a)$};
%  \node[xshift=9.49cm, yshift=-2.5cm] {$(b)$};
}

==> bn-unrooted.tex <==
\input{rooted_tree}
\tikzstyle{fakenode} = [obs, fill=gray!10, draw=gray, densely dashed]
\tikz[scale=0.75]{
  \begin{scope}[xscale=0.45, yscale=0.45, transform shape]
%  \node[xshift=3cm] (UTR) {};
%  \node[left=of UTR, xshift=-0.5cm] (UTL) {};
%  \node[leaf, right=of UTR, xshift=-0.6cm, yshift=2cm] (UTB) {$B$};
%  \node[leaf, right=of UTR, xshift=-0.6cm, yshift=-2cm] (UTD) {$D$};
%  \node[leaf, left=of UTL, xshift=0.6cm, yshift=2cm] (UTA) {$A$};
%  \node[leaf, left=of UTL, xshift=0.6cm, yshift=-2cm] (UTC) {$C$};
%  
%  \undiredgeleaf[thick] {UTR}{UTB, UTD} ;
%  \undiredgeleaf[>={}, thick] {UTL}{UTA, UTC};
%  \undiredge[thick]{UTR}{UTL};
  \node[xshift=1.5cm, yshift=-2.5cm] (UTUp) {};
  \node[below=of UTUp, yshift=-0.25cm] (UTDown) {};
  \node[leaf, above=of UTUp, xshift=-1.5cm, yshift=-0.75cm] (UTA) {\scalebox{1.4}{$A$}};
  \node[leaf, above=of UTUp, xshift=1.5cm, yshift=-0.75cm] (UTB) {\scalebox{1.4}{$B$}};
  \node[leaf, below=of UTDown, xshift=-1.5cm, yshift=0.75cm] (UTC) {\scalebox{1.4}{$C$}};
  \node[leaf, below=of UTDown, xshift=1.5cm, yshift=0.75cm] (UTD) {\scalebox{1.4}{$D$}}; 
  \undiredgeleaf[thick]{pos=0.6, below=1pt, font=\Large}{1}{UTUp}{UTA}
  \undiredgeleaf[thick]{pos=0.6, below=1pt,font=\Large}{2}{UTUp}{UTB};
  \undiredgeleaf[thick]{pos=0.6, above=2pt,font=\Large}{4}{UTDown}{UTC};
  \undiredgeleaf[thick]{pos=0.6, above=2pt,font=\Large}{5}{UTDown}{UTD};
  \undiredge[thick]{pos=0.5, right=1pt,font=\Large}{3}{UTUp}{UTDown};
  \end{scope}
  
  \begin{scope}[xscale=0.45, yscale=0.45, transform shape, xshift=9cm]
  \node[leaf, xshift=5cm, yshift=2cm] (T1A){\scalebox{1.4}{$A$}};
  \node[leaf, below=of T1A, yshift=1.3cm] (T1B) {\scalebox{1.4}{$B$}};
  \node[leaf, below=of T1B, yshift=1.3cm] (T1C) {\scalebox{1.4}{$C$}};
  \node[leaf, below=of T1C, yshift=1.3cm] (T1D) {\scalebox{1.4}{$D$}};
  \node[left = of T1C, xshift=-0.6cm, yshift=-0.7cm] (T1S3) {};
  \node[left = of T1S3, xshift=0.5cm, yshift=1.05cm] (T1S2) {};
  \node[left = of T1S2, xshift=0.5cm, yshift=1.15cm] (T1S1) {};
  \node[left = of T1S1, xshift=0.75cm, font=\Large] (T1root) {$1$};
  
  \node[left=of T1root, xshift=-2.5cm, yshift=-1.1cm] (T1Arrow) {};
  \path (T1Arrow) edge[<->, >= stealth, thick] node[pos=0.5, above=4pt, font=\LARGE, sloped]{root/unroot} +(1.3, 0.75);
  
  \csquaredgeleaf[thick] {T1S3} {T1C, T1D};
  \csquaredgeleaf[thick] {T1S2} {T1B};
  \csquaredge[thick] {T1S2}{T1S3};
  \csquaredgeleaf[thick] {T1S1} {T1A};
  \csquaredge[thick] {T1S1} {T1S2};
  \draw[thick] (T1root) -- (T1S1.center);  
  
%  \node[left=of T1root, xshift=-0.5cm, yshift=-4cm] (LArrow) {};
%  \path (LArrow) edge[->, >= stealth, thick] node[pos=0.5, above=2pt, font=\large]{rooting} +(1.0, 0);
  
  
  \node[leaf, below=of T1D, yshift=0.8cm] (T2A){\scalebox{1.4}{$A$}};
  \node[leaf, below=of T2A, yshift=1.3cm] (T2B) {\scalebox{1.4}{$B$}};
  \node[leaf, below=of T2B, yshift=1.3cm] (T2C) {\scalebox{1.4}{$C$}};
  \node[leaf, below=of T2C, yshift=1.3cm] (T2D) {\scalebox{1.4}{$D$}};
  \node[left = of T2A, xshift=-1.4cm, yshift=-0.7cm] (T2S3) {};
  \node[left = of T2C, xshift=-1.4cm, yshift=-0.7cm] (T2S2) {};
  \node[left = of T2S2, xshift=0.5cm, yshift=1.25cm] (T2S1) {};
  \node[left = of T2S1, xshift=0.75cm, font=\Large] (T2root) {$3$};
  
  \node[left=of T2root, xshift=-2.5cm, yshift=0.8cm] (T2Arrow) {};
  \path (T2Arrow) edge[<->, >=stealth, thick] node[pos=0.5, below=1pt, font=\LARGE, sloped]{root/unroot} +(1.3,-0.75);
  
  \csquaredgeleaf[thick]{T2S3}{T2A, T2B};
  \csquaredgeleaf[thick]{T2S2}{T2C, T2D};
  \csquaredge[thick]{T2S1}{T2S2, T2S3};
  \draw[thick] (T2root) -- (T2S1.center);
  \end{scope}
  
  \begin{scope}[xscale=0.45, yscale=0.45, transform shape, xshift=20cm]
  \node[fakenode, xshift=6cm, yshift=2cm] (N1S4){\scalebox{1.8}{$A$}};
  \node[fakenode, xshift=6cm, yshift=0.6cm] (N1S5) {\scalebox{1.8}{$A$}};
  \node[fakenode, xshift=6cm, yshift=-0.8cm] (N1S6) {\scalebox{1.8}{$B$}};
  \node[obs, xshift=6cm, yshift=-2.2cm] (N1S7) {\scalebox{1.2}{$\dfrac{C}{D}$}}; 
  
 \node[fakenode, left= of N1S4, xshift=-0.5cm, yshift=-1cm] (N1S2) {\scalebox{1.8}{$A$}};
 \node[obs, below = of N1S2, yshift=-0.12cm] (N1S3) {\scalebox{1.2}{$\dfrac{B}{CD}$}};
 \node[obs, left= of N1S2, xshift=-0.2cm, yshift=-1cm] (N1S1) {\scalebox{1.2}{$\dfrac{A}{BCD}$}};
 
 \node[left=of N1S1, xshift=-2.5cm] (N1Arrow) {};
 \path (N1Arrow) edge[<->, >=stealth, thick] +(1.5,0);
 
 \annotatededge[densely dashed, gray!50]{pos=0.4, above=2pt}{}{N1S2}{N1S4, N1S5};
 \annotatededge[densely dashed, gray!50]{pos=0.4, above=2pt}{}{N1S3}{N1S6};
 \edge{N1S3}{N1S7};
 \annotatededge[densely dashed, gray!50]{pos=0.4, above=2pt}{}{N1S1}{N1S2};
 \edge{N1S1}{N1S3};
  
  \node[fakenode, xshift=6cm, yshift=-4.4cm] (N2S4){\scalebox{1.8}{$A$}};
  \node[fakenode, xshift=6cm, yshift=-5.8cm] (N2S5) {\scalebox{1.8}{$B$}};
  \node[fakenode, xshift=6cm, yshift=-7.2cm] (N2S6) {\scalebox{1.8}{$C$}};
  \node[fakenode, xshift=6cm, yshift=-8.6cm] (N2S7) {\scalebox{1.8}{$D$}}; 
  
 \node[obs, left= of N2S4, xshift=-0.5cm, yshift=-1cm] (N2S2) {\scalebox{1.2}{$\dfrac{A}{B}$}};
 \node[obs, below = of N2S2, yshift=-0.08cm] (N2S3) {\scalebox{1.2}{$\dfrac{C}{D}$}};
 \node[obs, left= of N2S2, xshift=-0.2cm, yshift=-1cm] (N2S1) {\scalebox{1.2}{$\dfrac{AB}{CD}$}};
 
  \node[left=of N2S1, xshift=-2.5cm] (N2Arrow) {};
 \path (N2Arrow) edge[<->, >=stealth, thick] +(1.5,0);
 
 \annotatededge[densely dashed, gray!50]{pos=0.4, above=2pt}{}{N2S2}{N2S4, N2S5};
 \annotatededge[densely dashed, gray!50]{pos=0.4, above=2pt}{}{N2S3}{N2S6, N2S7};
 \edge{N2S1}{N2S2, N2S3};
 
 \node[right=of N1S5, xshift=1.75cm, yshift=-0.7cm] (N1Arrowout) {};
 \path (N1Arrowout) edge[<->, >=stealth, thick] +(1.3,-0.75);
 \node[right=of N2S6, xshift=1.75cm, yshift=0.7cm] (N2Arrowout) {};
 \path (N2Arrowout) edge[<->, >=stealth, thick] +(1.3,0.75);
 \end{scope}
% 
 \begin{scope}[xscale=0.6, yscale=0.6, transform shape, xshift=25.5cm, yshift=.5cm]
%   \foreach \x/\xtext/\xname in {-1/UNS4/S_4, -2.5/UNS5/S_5, -4/UNS6/S_6, -5.5/UNS7/S_7} {
%    \node[obs, below=of UTD, yshift=\x cm] (\xtext){$\xname$};
%    };
  \node[obs, xshift=4cm, yshift=0cm] (UNS4) {\scalebox{1.6}{$S_4$}};
  \node[obs, xshift=4cm, yshift=-2cm] (UNS5) {\scalebox{1.6}{$S_5$}};
  \node[obs, xshift=4cm, yshift=-4cm] (UNS6) {\scalebox{1.6}{$S_6$}};
  \node[obs, xshift=4cm, yshift=-6cm] (UNS7) {\scalebox{1.6}{$S_7$}};
  
  \node[obs, left=of UNS4, xshift=-0.5cm, yshift=-1.6cm] (UNS2) {\scalebox{1.6}{$S_2$}};
  \node[obs, below=of UNS2, yshift=-0.95cm] (UNS3) {\scalebox{1.6}{$S_3$}};
  \node[latent, left=of UNS2, xshift=-0.2cm, yshift=-1.4cm] (UNS1) {\scalebox{1.6}{$S_1$}};
  
  \edge {UNS2}{UNS4, UNS5};
  \edge {UNS3}{UNS6, UNS7};
  \edge {UNS1}{UNS2, UNS3};
 \end{scope}
% \node[xshift=0.55cm, yshift=-3.5cm] {$(a)$};
% \node[xshift=4.2cm, yshift=-3.5cm] {$(b)$};
% \node[xshift=8.1cm, yshift=-3.5cm] {$(c)$};
% \node[xshift=12.3cm, yshift=-3.5cm] {$(d)$};
}

==> rooted_tree.tex <==

% Clade node
\tikzstyle{clade} = [latent, rectangle, minimum size=18pt, node distance=2]

% Leaf node
\tikzstyle{leaf} = [font=\fontsize{15}{15}\selectfont, node distance=2]

% \squaredge  [options]  {inputs}  {outputs}
\newcommand{\squaredge}[3][] {
  % Connect all nodes #2 to all node #3.
  \foreach \x in {#2} {
    \foreach \y in {#3} {
      \draw[semithick, #1]  (\x) -- (\x |- \y) -- (\y);
    };
  };
}

% \csquaredge [options] {inputs} {outputs}
\newcommand{\csquaredge}[3][] {
  % Connect all nodes #2 to all node #3.
  \foreach \x in {#2} {
    \foreach \y in {#3} {
      \draw[semithick, #1]  (\x.center) -- (\x |- \y) -- (\y.center);
    };
  };
}

\newcommand{\undiredge}[5][] {
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#4} {
    \foreach \y in {#5} {
      \path (\x.center) edge[#1] node[pos=0.5, below, #2]{#3} (\y.center);
      };
    };
}

\newcommand{\undiredgeleaf}[5][] {
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#4} {
    \foreach \y in {#5} {
      \path (\x.center) edge[#1]node[pos=0.5, below, #2]{#3} (\y);
      };
    };
}


% \csquaredgeleaf [options] {inputs} {outputs}
\newcommand{\csquaredgeleaf}[3][] {
  % Connect all nodes #2 to all node #3.
  \foreach \x in {#2} {
    \foreach \y in {#3} {
      \draw[semithick, #1]  (\x.center) -- (\x |- \y) -- (\y);
    };
  };
}

% \annotatededge [options] [options] {edge value} {inputs} {outputs}
\newcommand{\annotatededge}[5][] {
 % Connect all nodes #2 to all node #3
 \foreach \x in {#4} {
   \foreach \y in {#5} {
     \path (\x) edge [->, >={triangle 45}, #1] node [pos=0.5, below, #2] {#3} (\y);
     };
   };

}
      


